QT-DoG: Quantization-aware Training for Domain Generalization

A key challenge in Domain Generalization (DG) is preventing overfitting to source domains, which can be mitigated by finding flatter minima in the loss landscape. In this work, we propose Quantization-aware Training for Domain Generalization (QT-DoG) and demonstrate that weight quantization effectively leads to flatter minima in the loss landscape, thereby enhancing domain generalization. Unlike traditional quantization methods focused on model compression, QT-DoG exploits quantization as an implicit regularizer by inducing noise in model weights, guiding the optimization process toward flatter minima that are less sensitive to perturbations and overfitting. We provide both an analytical perspective and empirical evidence demonstrating that quantization inherently encourages flatter minima, leading to better generalization across domains. Moreover, with the benefit of reducing the model size through quantization, we demonstrate that an ensemble of multiple quantized models further yields superior accuracy than the state-of-the-art DG approaches with no computational or memory overheads. Code is released at: https://saqibjaved1.github.io/QT_DoG/.

==> Tables/Indomain.tex <==

\bgroup
\def\arraystretch{0.9}
\begin{table}[t]
\begin{center}
\scalebox{0.95}{

% \caption{\small \textbf{Comparison between generalization methods on \data{PACS}.} The scores are averaged over all settings using different target domains. \greenp{$\uparrow$} and \redp{$\downarrow$} indicate statistically significant improvement and degradation from ERM.}

% \resizebox{\linewidth}{!} {
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|c|c|c}
% \tiny
\toprule
\textbf{Method}&  \textbf{In-domain} & \textbf{Out-domain} & \textbf{Compression} \\
\midrule
        \midrule

ERM &        96.6 $\pm$ 0.2 & 90.1 $\pm$ 0.2 & -\\

SAM &       97.4 $\pm$ 0.1 & 90.8 $\pm$ 0.1  & -\\
SWA &       97.1 $\pm$ 0.1 &  90.7 $\pm$ 0.1 & -\\

SMA &        96.8 $\pm$ 0.2  &  90.7 $\pm$ 0.4 & - \\
SWAD &       97.7 $\pm$ 0.2  &  90.8 $\pm$ 0.3 & -  \\
\rowcolor{Gray}
QT-DoG &        97.3 $\pm$ 0.2 &  91.1 $\pm$ 0.2 & $\sim$4.6x \\
        \hline

\bottomrule

\end{tabular}
}
\end{center}
\caption{\footnotesize\textbf{Comparison between generalization methods on PACS for IID settings.} We report the accuracy averaged across all domains of the PACS dataset. Our proposed approach is shaded in Gray.}
\label{IID}
% \vspace{-2em}
\end{table}
\egroup


ERM (our runs)&        90.1 $\pm$ 0.2 & 47.2 $\pm$ 0.2 & -\\
SMA~\cite{arpit2021ensemble} &       90.7 $\pm$ 0.4  &  50.3 $\pm$ 0.5 & -  \\
SWAD~\cite{cha2021swad} &       90.8 $\pm$ 0.3  &  50.4 $\pm$ 0.4 & -  \\
\rowcolor{Gray}
QT-DoG &        91.1 $\pm$ 0.2 &  50.8  $\pm$ 0.3 & $\sim$4.6x \\
        \hline

==> Tables/LSQ_swisscube_rebuttal.tex <==
\bgroup
\def\arraystretch{1.2}
\begin{table}[t]
	\centering
	\scalebox{0.80}{
	% \begin{tabular}{lcccc!{\vrule width 1pt}cccc}
	\begin{tabular}{c|c|c}
 
	\toprule
	   Quantization Mode   & {ADI-0.1d}  & Compression \\
	\midrule
        LSQ          & 71.2 & 8x   \\
        \textbf{MQ (ours)} & \textbf{81.1} & \textbf{8.2x} 	\\
	\bottomrule
	\end{tabular}
	}
 \vspace{1.5mm}
 \caption{\textbf{Quantization of WDR on the Swisscube dataset}.
}
 %with different compression factors.
\label{tab:lsqswiss} 
\vspace{-7mm}
\end{table}
\egroup

==> Tables/copy_main.tex <==
% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
%     \hline
%         ~ & PACS & VLCS & Office & Terra & DomainNet & Avg \\ \hline
%         ERM & ~ & ~ & ~ & ~ & ~ & 64  \\ \hline
%         Miro & 85.4 ± 0.4 & 79.0 ± 0. & 70.5 ± 0.4 & 50.4 ± 1.1 & 44.3 ± 0.2 & 65.9 \\ \hline
%         SWAD & 88.1 ± 0.4 & 79.1 ± 0.4 & 70.6 ± 0.3 & 50.0 ± 0.4 & 46.5 ± 0.2 & 66.9 \\ \hline
        
%         EOA & 88.6 & 79.1 & 72.5 & 52.3 & 47.4 & 67.98\\ \hline
%         EOQ & 89.3 & 79.3 & 71.7 & 53.2 & 47.9 & 68.28  \\ \hline
%     \end{tabular}
% \end{table}
\noindent
\bgroup
\def\arraystretch{1.1}
\begin{table*}[!tbh]
\begin{center}
\scalebox{0.95}{
% \vspace{-12pt}

% \fontsize{9}{9}\selectfont

\begin{tabular}{l|c|l@{\hspace{0.18cm}}l@{\hspace{0.18cm}}l@{\hspace{0.18cm}}l@{\hspace{0.18cm}}l|l}
\hline
{Algorithm} &   M      & {PACS}           & {VLCS}           & {Office}  & {TerraInc} & {DomainNet}      & {Avg}. \\ \hhline{=======|=}
\multicolumn{8}{c}{{ResNet-50 (25M Parameters, Pre-trained on ImageNet)}}\\
\hline



ERM \cite{gulrajani2020search} & 1& 85.5 $\pm$ 0.5 & 77.4 $\pm$ 0.3 & 67.5 $\pm$ 0.5 & 47.2 $\pm$ 0.4 & 41.2 $\pm$ 0.2 & 63.8\\ 
IRM \cite{arjovsky2019invariant}& 1 & 84.4 $\pm$ 1.1            & 78.1 $\pm$ 0.0            & 66.6 $\pm$ 1.0            & 47.9 $\pm$ 0.7            & 35.7 $\pm$ 1.9 & 62.5\\
Group DRO \cite{Sagawa2020Distributionally}& 1  & 84.1 $\pm$ 0.4            & 77.2 $\pm$ 0.6            & 66.9 $\pm$ 0.3            & 47.0 $\pm$ 0.3            & 33.7 $\pm$ 0.2 & 61.8\\
Mixup \cite{xu2020adversarial,wang2020heterogeneous}&  1 & 84.3 $\pm$ 0.5            & 77.7 $\pm$ 0.4            & 69.0 $\pm$ 0.1            & 48.9 $\pm$ 0.8            & 39.6 $\pm$ 0.1 & 63.9\\
MLDG  \cite{li2018learning}&  1  & 84.8 $\pm$ 0.6            & 77.1 $\pm$ 0.4            & 68.2 $\pm$ 0.1            & 46.1 $\pm$ 0.8            & 41.8 $\pm$ 0.4 & 63.6\\
CORAL  \cite{sun2016deep}& 1  & 86.0 $\pm$ 0.2            & 77.7 $\pm$ 0.5            & 68.6 $\pm$ 0.4            & 46.4 $\pm$ 0.8            & 41.8 $\pm$ 0.2 & 64.1\\
MMD   \cite{li2018domain}& 1 & 85.0 $\pm$ 0.2            & 76.7 $\pm$ 0.9            & 67.7 $\pm$ 0.1            & 49.3 $\pm$ 1.4            & 39.4 $\pm$ 0.8 & 63.6\\
DANN \cite{ganin2016domain}& 1 & 84.6 $\pm$ 1.1            & 78.7 $\pm$ 0.3            & 65.4 $\pm$ 0.6            & 48.4 $\pm$ 0.5            & 38.4 $\pm$ 0.0 & 63.1\\
C-DANN  \cite{li2018deep}& 1 & 82.8 $\pm$ 1.5            & 78.2 $\pm$ 0.4            & 65.6 $\pm$ 0.5            & 47.6 $\pm$ 0.8            & 38.9 $\pm$ 0.1 & 62.6\\

Fish \cite{shi2022gradient}&  1  & 85.5 $\pm$ 0.3 & 77.8 $\pm$ 0.3 & 68.6 $\pm$ 0.4 & 45.1 $\pm$ 1.3 & 42.7 $\pm$ 0.2 & 63.9\\
Fishr \cite{rame_fishr_2021}&  1   & 85.5 $\pm$ 0.4 & 77.8 $\pm$ 0.1 & 67.8 $\pm$ 0.1 & 47.4 $\pm$ 1.6 & 41.7 $\pm$ 0.0 & 65.7\\
SWAD \cite{cha2021swad}&  1   & 88.1 $\pm$ 0.4 & \underline{79.1 $\pm$ 0.4} & 70.6 $\pm$ 0.3 & 50.0 $\pm$ 0.4 & 46.5 $\pm$ 0.2 & 66.9\\
MIRO \cite{cha2022miro}&   1  & 85.4 $\pm$ 0.4 & 79.0 $\pm$ 0.0 & 70.5 $\pm$ 0.4 & 50.4 $\pm$ 1.1 & 44.3 $\pm$ 0.2 & 65.9\\
ARM$^\dagger$~\cite{zhang2022arm}&   1   & 85.1          & 77.6          & 64.8                & 45.5              & 35.5               & 61.7           \\
VREx$^\dagger$~\cite{krueger2020vrex}&   1  & 84.9          & 78.3          & 66.4                & 46.4              & 33.6               & 61.9           \\
RSC$^\dagger$~\cite{huang2020self}&  1    & 85.2          & 77.1          & 65.5                & 46.6              & 38.9               & 62.7           \\
Mixstyle$^\dagger$~\cite{zhou2021mixstyle}&  1    & 85.2          & 77.9          & 60.4                & 44.0              & 34.0               & 60.3           \\
SagNet$^\dagger$~\cite{nam2019sagnet}&  1   & 86.3          & 77.8          & 68.1                & 48.6              & 40.3               & 64.2           \\
ERM Ens. $^\dagger$\cite{arpit2021ensemble}&   6   & 87.6             & 78.5           &       70.8         & 49.2           &          \underline{47.7}      &   66.8   \\

DIWA$^\dagger$ \cite{rame2022diverse}& 60  &\underline{89.0}  & 78.6 & 72.8 & 51.9 & \underline{47.7} & \underline{68.0}  \\

EoA$^\dagger$\cite{arpit2021ensemble}&    6    & 88.6           & \underline{79.1}           & \textbf{72.5}          & \underline{52.3}           &        {47.4}        & \underline{68.0}\\
\rowcolor{Gray}
\hline
QT-DoG (ours)&  1  & 87.8$\pm$ 0.3 & 78.4$\pm$ 0.4 & 68.9$\pm$ 0.6 & 50.8$\pm$ 0.2 & 45.1$\pm$0.9 & 66.2 \\ 
\rowcolor{Gray}
EoQ(ours)&   5    & \textbf{89.3} & \textbf{79.3} & \underline{71.7} & \textbf{53.2} & \textbf{47.9} & \textbf{68.3}  \\ \hline

\hline
\end{tabular}
}
\end{center}

\caption{\footnotesize\textbf{Comparison with domain generalization methods.} Performance benchmarking on 5 datasets of the DomainBed benchmark. Highest accuracy is shown in bold, while second best is underlined. $^\dagger$ do not report confidence interval and ensembles do not have confidence interval because an ensemble uses all the models to make a prediction. Our proposed method is colored in Gray. Average accuracies and standard errors are reported from three trials. For all the reported results, we use the same training-domain validation protocol as \cite{gulrajani2020search}. $M$ corresponds to the number of models trained during training.}
\label{tab:benchmark}
% \vspace{-3em}
\end{table*}
\egroup


==> Tables/different_quant.tex <==


\bgroup
\def\arraystretch{1.0}

\begin{table}[t]
\begin{center}
\scalebox{0.9}{
\begin{tabular}{l|c|c|c}
\toprule
{\textbf{Quantization}} &\textbf{Type} & \textbf{In-domain} & \textbf{Out-domain} \\
\midrule
\midrule

No quant & - & 96.6 $\pm$ 0.2  &  84.7 $\pm$ 0.5   \\

OBC & PTQ & 96.8 $\pm$ 0.2  &  83.7 $\pm$ 0.4   \\
INQ & QAT & 97.1 $\pm$ 0.2  &  87.4 $\pm$ 0.3   \\
LSQ & QAT & \textbf{97.3 $\pm$ 0.2}  &  \textbf{87.8 $\pm$ 0.3}   \\

% \hline
% ERM+ Quant(8)& 4x &  97.0 $\pm$ 0.1  & 85.0 $\pm$ 0.1 & 90.9 $\pm$ 0.2 \\
% \rowcolor{Gray}
% ERM+ Quant(7)&  4.6x & \textbf{97.3 $\pm$ 0.2}    & \textbf{87.8 $\pm$ 0.3} 
%  & \textbf{92.3 $\pm$ 0.2}   \\

% ERM+ Quant(6) &  5.3x  &    97.1 $\pm$ 0.1  &  86.5 $\pm$ 0.1 & 91.1 $\pm$ 0.0    \\
% ERM+ Quant(5) & 6.4x & 97.0   $\pm$ 0.1   & 85.3 $\pm$ 0.4 & 91.0 $\pm$ 0.1   \\
%         \hline

\midrule
\bottomrule

\end{tabular}
}
\end{center}
\caption{\textbf{Model quantization with different quantization algorithms.} We report the average target domain accuracy and the average source domain accuracy across all domains in PACS~\cite{li2017deeper}. All the experiments are with 7 bit quantization.}
\label{different_quant}
\end{table}
\egroup

==> Tables/indomain_terra.tex <==

\bgroup
\def\arraystretch{0.9}
\begin{table}[!tbh]
\begin{center}
\scalebox{0.95}{

% \caption{\small \textbf{Comparison between generalization methods on \data{PACS}.} The scores are averaged over all settings using different target domains. \greenp{$\uparrow$} and \redp{$\downarrow$} indicate statistically significant improvement and degradation from ERM.}

% \resizebox{\linewidth}{!} {
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|c|c|c}
% \tiny
\toprule
\textbf{Algorithm}&  \textbf{In-domain} & \textbf{Out-domain} & \textbf{Compression} \\
\midrule
        \midrule

ERM (our runs)&        90.1 $\pm$ 0.2 & 47.2 $\pm$ 0.2 & -\\
SMA~\cite{arpit2021ensemble} &       90.7 $\pm$ 0.4  &  50.3 $\pm$ 0.5 & -  \\
SWAD~\cite{cha2021swad} &       90.8 $\pm$ 0.3  &  50.4 $\pm$ 0.4 & -  \\
\rowcolor{Gray}
QT-DoG &        91.1 $\pm$ 0.2 &  50.8  $\pm$ 0.3 & $\sim$4.6x \\
        \hline

\bottomrule

\end{tabular}
}
\end{center}
\caption{\footnotesize\textbf{Comparison between Generalization methods on Terra for IID settings.} We report the accuracy averaged across all domains of the Terra dataset. Our proposed approach is shaded in Gray.}
\label{IID_terra}
% \vspace{-4em}
\end{table}
\egroup


==> sec/0_abstract.tex <==
\begin{abstract}
Domain Generalization (DG) aims to train models that excel not only within the training (source) domain but also in novel, unseen (target) data distributions. An effective strategy is to introduce a regularization that favors finding a flatter minimum in the loss landscape, thus preventing overfitting to the source domains. In this paper, we show that weight quantization incurs such a regularizing effect. Thus, we introduce a novel method, Quantization-Aware Training for Domain Generalization (QT-DoG), demonstrating that reducing the bit-precision of the network weights can indeed enhance its generalization capabilities. Furthermore, with the benefit of reducing the model size through quantization, we demonstrate that an ensemble of multiple quantized models further yields superior accuracy than the state-of-the-art DG approaches without computational or memory overheads.

\keywords{Domain Generalization, Quantization, Regularization, Ensemble, Network Compression, Flat Minima}


\end{abstract}
